An Efficient Matrix Multiplication Algorithm for Accelerating Inference in Binary and Ternary Neural Networks

Despite their tremendous success and versatility, Deep Neural Networks (DNNs) such as Large Language Models (LLMs) suffer from inference inefficiency and rely on advanced computational infrastructure. To address these challenges and make these models more accessible and cost-effective, in this paper, we propose algorithms to improve the inference time and memory efficiency of DNNs with binary and ternary weight matrices. Particularly focusing on matrix multiplication as the bottleneck operation of inference, we observe that, once trained, the weight matrices of a model no longer change. This allows us to preprocess these matrices and create indices that help reduce the storage requirements by a logarithmic factor while enabling our efficient inference algorithms. Specifically, for a $n\times n$ weight matrix, our efficient algorithm guarantees a time complexity of $O(\frac{n^2}{\log n})$, a logarithmic factor improvement over the standard vector-matrix multiplication. Besides theoretical analysis, we conduct extensive experiments to evaluate the practical efficiency of our algorithms. Our results confirm the superiority of our approach both with respect to time and memory, as we observed a reduction in the multiplication time up to 29x and memory usage up to 6x. When applied to LLMs, our experiments show up to a 5.24x speedup in the inference time.

==> init.tex <==
\section{Introduction}
TBD!

1.58bit LLMs: \href{https://arxiv.org/abs/2402.17764}{https://arxiv.org/abs/2402.17764}

\section{Problem}
Given a vector $v$ of size $n$ and a matrix $A$ of size $n \times n$ such that all elements {\bf of the matrix} are in $\{+1, 0, -1\}$, find the product $v \cdot A$ efficiently.\footnote{Better than $O(n^2)$!} $A$ contains $n$ columns $\{c_1, c_2, ..., c_n\}$.

\subsection{Observation 1}
Each matrix $A$ can be written as the subtraction of two matrices $A_1$ and $A_2$ such that both $A_1$ and $A_2$ have only $\{+1, 0\}$ elements.

\[
A = A_1 - A_2
\]

\subsection{Problem 2}
Now, we can reduce Problem 1 to calculating a product $v \cdot A$ such that $A$ only has elements in $\{+1, 0\}$.

\subsection{Permutation Method (Algorithm I)}
Focus on the first two columns $c_1$ and $c_2$. Each element is either +1 or 0. Let a pair $(c_1[i], c_2[i])$ denote two elements from each of these vectors in front of each other. There are 4 cases for $(c_1[i], c_2[i])$:

\begin{itemize}
    \color{red}{\item $(c_1[i], c_2[i]) = (0, 0)$}
    \color{blue}{\item $(c_1[i], c_2[i]) = (0, +1)$}
    \color{olive}{\item $(c_1[i], c_2[i]) = (+1, 0)$}
    \color{brown}{\item $(c_1[i], c_2[i]) = (+1, +1)$}
\end{itemize}


Define a permutation $\pi_2$ that permutes both $c_1$ and $c_2$ such that we have all $(0, 0)$ at the beginning, then all $(0, +1)$, and so on. For example, let

\begin{align}
c_1 = 
\begin{pmatrix}
  +1 \\
  0 \\
  0 \\
  +1 \\
  +1 \\
  0
\end{pmatrix}, \quad
c_2 = \begin{pmatrix}
  0 \\
  +1 \\
  0 \\
  0 \\
  +1 \\
  0
\end{pmatrix}
\end{align}

Then, the permutated vectors is like this:

\begin{align}
    \pi_2(c_1) = 
    \begin{pmatrix}
        \color{red}{0} \\
        \color{red}{0} \\
        \color{blue}{0} \\
        \color{olive}{+1} \\
        \color{olive}{+1} \\
        \color{brown}{+1}
    \end{pmatrix}, \quad
    \pi_2(c_2) = 
    \begin{pmatrix}
        \color{red}{0} \\
        \color{red}{0} \\
        \color{blue}{+1} \\
        \color{olive}{0} \\
        \color{olive}{0} \\
        \color{brown}{+1}
    \end{pmatrix}
\end{align}

Now, we can generalize this permutation to a set of $k \leq \log(n)$ columns. Putting all $(0, 0, \cdots, 0)$ at the beginning, then $(0, 0, \cdots, 0, +1)$ after that, and so on. Then $(+1, +1, \cdots, +1)$ at the end.

Define a segment as a set of consecutive elements of a vector that all have the same value. For example, in the above, $\pi_2(c_1)$ and $\pi_2(c_2)$ both have 4 segments (colors). Let $I_{i, j}$ denote the $i^{th}$ segment of $j^{th}$ column ($i \leq 2^k$ and $j \leq k$). In other words, each column would have at most $2^k$ segments.

\begin{align}
[I_{i, j}] =
    \begin{bmatrix}
      0 & 0 & \cdots & 0 \\
      0 & 0 & \cdots & +1 \\
      \vdots & \vdots & \ddots & \vdots \\
      +1 & +1 & \cdots & +1
    \end{bmatrix}_{2^k \times k}
\end{align}

\begin{lemma}
    We can calculate the product $v \cdot A[c_1 \mid c_2 \mid \cdots \mid c_K]$ in $O(n + k \cdot 2^k)$.
\end{lemma}
\begin{proof}
    TODO
\end{proof}

Using the above lemma one can calculate $v \cdot A$ in $O(\frac{n}{k} \cdot (n + k\cdot2^k))$.

\paragraph{Observation} As a result, we should find largest $k$ such that:

\[
k \cdot 2^k = O(n)
\]
Then, {\bf the running time is $O(n^2 / k)$}.

Example: $k = \log(\frac{n}{\log(n)}) = \log(n) - \log(\log(n))$

\subsection{Algorithm II (Improvement)}
Given a vector of size $2^k$ and the binary encoded matrix of size $2^k \times k$, we can calculate the product in $O(n + 2^k)$ instead of $O(n + k \cdot 2^k)$

\subsubsection{How?}
Start from the $k^{th}$ column. We can calculate $r[k]$ in $O(2^k)$. Where $r$ is the response of size $k$. This can be done by one iteration through $v$. During this iteration, also create a vector $v_2$ that is $2^{k-1}$ long, and each element is the sum of two consecutive elements of $v$.

Now to calculate $r[k - 1]$, we can just iterate $v_2$ once. This can be done in $O(2^{k - 1})$. During this iteration also create $v_3$ which is $2^{k - 2}$ long and each element is the sum of two consecutive elements of $v_2$. 

Continuing this process would result in calculating $r$ in $\sum^{k}_{i = 1} 2^k$ time which is $O(2^k)$.

The reason that $r[k - i]$ can be calculated by one iteration through $v_{i}$ is that in the $(k - i)^{th}$ column just has consecutive 0s and 1s of size $2^i$.

\paragraph{Note:} The running time of Algorithm II is $O(\frac{n^2}{\log(n)})$.

\begin{algorithm}[!tb]
    \caption{Algorithm II}
    \begin{algorithmic}[1] \small
    \Require{An input vector $v$ of size $2^k$, the binary encoded matrix A of size $2^k \times k$}
    \Ensure{Calculate $v \cdot A$ in time of $O(2^k)$}
    \Function{Alg2}{$v, A$}
        \State $result \gets \vec{0}$\Comment{Initialize with $\vec{0}$ vector}
        \State $v_{k} \gets v$
        \For{$i$ from $k$ to $1$}
        \State $result[i] \gets \text{OddSum}(v_i)$\Comment{$O(|v_i|)$}
        \State $v_{i - 1} \gets \text{Compact}(v_i)$\Comment{$O(|v_i|)$}
        \State 
        \EndFor
        \State {\bf Return} $result$\Comment{Vector of size $k$}
    \EndFunction
    \Statex
    \Function{OddSum}{$v$}\Comment{Sum the odd elements: $O(|v|)$}
    \State $sum \gets 0$
    \For{$i \leq |v|$}
    \If{$i$ is odd}
    \State $sum \gets res + v[i]$
    \EndIf
    \EndFor
    \State {\bf Return} $sum$
    \EndFunction

    \Function{Compact}{$v$}\Comment{Add each two consecutive elements}
    \State $v^{\prime} \gets \vec{0}$\Comment{Vector of size $\frac{|v|}{2}$}
    \For{$i \leq \frac{|v|}{2}$}
    \State $v^{\prime}[i] \gets v[2 i] + v[2 i + 1]$
    \EndFor
    \State {\bf Return} $v^{\prime}$ \Comment{$v^{\prime} = \frac{|v|}{2}$}
    \EndFunction
    
    \end{algorithmic}
\end{algorithm}
